Rees coextensions of finite, negative tomonoids

A totally ordered monoid, or tomonoid for short, is a monoid endowed with a compatible total order. We deal in this paper with tomonoids that are finite and negative, where negativity means that the monoidal identity is the top element. Examples can be found, for instance, in the context of finite-valued fuzzy logic. By a Rees coextension of a negative tomonoid $S$, we mean a negative tomonoid $T$ such that a Rees quotient of $T$ is isomorphic to $S$. We characterise the set of all those Rees coextensions of a finite, negative tomonoid that are by one element larger. We thereby define a method of generating all such tomonoids in a stepwise fashion. Our description relies on the level-set representation of tomonoids, which allows us to identify the structures in question with partitions of a certain type.

==> tomtable.tex <==

\edef\tomtableIX{
    {0,t,u,v,w,x,y,z,1},
    {0,0,t,t,u,v,w,x,z},
    {0,0,0,0,t,t,u,v,y},
    {0,0,0,0,t,t,u,v,x},
    {0,0,0,0,0,0,t,t,w},
    {0,0,0,0,0,0,t,t,v},
    {0,0,0,0,0,0,0,0,u},
    {0,0,0,0,0,0,0,0,t},
    {0,0,0,0,0,0,0,0,0}}

\edef\tomtableVIII{
    {0,u,v,w,x,y,z,1},
    {0,0,0,u,v,w,x,z},
    {0,0,0,0,0,u,v,y},
    {0,0,0,0,0,u,v,x},
    {0,0,0,0,0,0,0,w},
    {0,0,0,0,0,0,0,v},
    {0,0,0,0,0,0,0,u},
    {0,0,0,0,0,0,0,0}}

\edef\tomtableVII{
    {0,v,w,x,y,z,1},
    {0,0,0,v,w,x,z},
    {0,0,0,0,0,v,y},
    {0,0,0,0,0,v,x},
    {0,0,0,0,0,0,w},
    {0,0,0,0,0,0,v},
    {0,0,0,0,0,0,0}}

\edef\tomtableVI{
    {0,w,x,y,z,1},
    {0,0,0,w,x,z},
    {0,0,0,0,0,y},
    {0,0,0,0,0,x},
    {0,0,0,0,0,w},
    {0,0,0,0,0,0}}

\edef\tomtableV{
    {0,x,y,z,1},
    {0,0,0,x,z},
    {0,0,0,0,y},
    {0,0,0,0,x},
    {0,0,0,0,0}}

\edef\tomtableIV{
    {0,y,z,1},
    {0,0,0,z},
    {0,0,0,y},
    {0,0,0,0}}

\edef\tomtableIII{
    {0,z,1},
    {0,0,z},
    {0,0,0}}

\edef\tomtableII{
    {0,1},
    {0,0}}

\edef\tomtableI{
    {1}}


